CCpdf: Building a High Quality Corpus for Visually Rich Documents from Web Crawl Data

In recent years, the field of document understanding has progressed a lot. A significant part of this progress has been possible thanks to the use of language models pretrained on large amounts of documents. However, pretraining corpora used in the domain of document understanding are single domain, monolingual, or nonpublic. Our goal in this paper is to propose an efficient pipeline for creating a big-scale, diverse, multilingual corpus of PDF files from all over the Internet using Common Crawl, as PDF files are the most canonical types of documents as considered in document understanding. We analysed extensively all of the steps of the pipeline and proposed a solution which is a trade-off between data quality and processing time. We also share a CCpdf corpus in a form or an index of PDF files along with a script for downloading them, which produces a collection useful for language model pretraining. The dataset and tools published with this paper offer researchers the opportunity to develop even better multilingual language models.

==> autozoil-extras.tex <==

\newcommand{\code}[1]{\texttt{#1}}
\newcommand{\noqa}[1]{}
\newcommand{\noqall}[1]{}



==> biographies.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images-michal_turski.jpg}}]{ MichaŁ Turski } received the B.S. degree in Robotics from the Warsaw University of Technology, Poland, in 2018, the B.S. degree in Computer Science from the Warsaw University of Technology, Poland, in 2019, and the M.S. degree in Computer Science from  Warsaw University of Technology, Poland, in 2020.
He is currently pursuing the Ph.D. degree. His research interests are in machine learning (ML), natural language processing (NLP), and structured data usage.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.35in,clip,keepaspectratio]{images-ts_img.jpeg}}]{Tomasz StanisŁawek} received the M.S. degree in computer science from the Warsaw School of Information Technology, Warsaw, Poland, under the auspices of the Polish Academy of Sciences, Warsaw. In 2022 he received the Ph.D. degree in machine learning from the Warsaw University of Technology. He is currently working as a Senior Research Scientist at Snowflake. His research interests include Natural Language Processing and machine learning applications.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images-kk_photo.jpg}}]{Karol Kaczmarek} received the M.S. degree in computer science from the Faculty of Mathematics and Computer Science, Adam Mickiewicz University, Poznan, Poland. From 2019 started the Ph.D. in Language Modeling area in the Faculty of Mathematics and Computer Science, Adam Mickiewicz University, Poznan, Poland. He is currently working in Snowflake as developer and machine learning integrator. His main research interest is Language Modeling, especially Language Modeling in the text.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images-pd_photo.jpg}}]{PaweŁ Dyda} received the M.S. degree in computer science from Polish-Japanese Academy of Information Technology, Warsaw, Poland in 2015. In 2020 he started the Industrial Ph.D. programme at the Faculty of Mathematics and Computer Science, Adam Mickiewicz University, Poznan, Poland. He is currently Research Scientist (machine learning) at Snowflake Inc. His research interests span Computer Vision, Information Extraction and Language Modeling.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images-fg_photo.jpg}}]{Filip GraliŃski} received the M.S. degree in computer science from Adam Mickiewicz University, Poznan, Poland and, in 2007, the Ph.D. degree in computational linguistics from Adam Mickiewicz University. He is currently working as a Principal Research Scientist at Snowflake and as a professor at Adam Mickiewicz University. His research interests include Natural Language Processing and evaluation of machine learning systems.
\end{IEEEbiography}


==> other-extras.tex <==


\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage[textsize=tiny]{todonotes}
\usepackage{graphicx}
\usepackage{booktabs}
\usepackage{latexsym}


\usepackage{footnote}
\makesavenoteenv{tabular}
\makesavenoteenv{table}
\makesavenoteenv{table*}


\usepackage{xurl}


\newcommand\minput[1]{%
  \input{#1}%
  \ifhmode\ifnum\lastnodetype=11 \unskip\fi\fi}

\usepackage{hyperref}
\usepackage{xstring}
\newcommand{\gonitoref}[1]{\{\href{https://gonito.net/q/#1}{\StrMid{#1}{1}{6}}\}}
\newcommand{\gonitobarescore}[1]{\minput{scores-#1.txt}}
\newcommand{\gonitoscore}[1]{\gonitobarescore{#1} \gonitoref{#1}}
\newcommand{\gonitoentry}[1]{\gonitoref{#1} & \minput{scores-#1.txt}}
\usepackage{multirow}


